An Experimental Study of Different Aggregation Schemes in Semi-Asynchronous Federated Learning

Federated learning is highly valued due to its high-performance computing in distributed environments while safeguarding data privacy. To address resource heterogeneity, researchers have proposed a semi-asynchronous federated learning (SAFL) architecture. However, the performance gap between different aggregation targets in SAFL remain unexplored. In this paper, we systematically compare the performance between two algorithm modes, FedSGD and FedAvg that correspond to aggregating gradients and models, respectively. Our results across various task scenarios indicate these two modes exhibit a substantial performance gap. Specifically, FedSGD achieves higher accuracy and faster convergence but experiences more severe fluctuates in accuracy, whereas FedAvg excels in handling straggler issues but converges slower with reduced accuracy.

==> contents/abstract.tex <==
\begin{abstract}
Federated learning is highly valued due to its high-performance computing in distributed environments while safeguarding data privacy. To address resource heterogeneity, researchers have proposed a semi-asynchronous federated learning (SAFL) architecture. However, the performance gap between different aggregation targets remains unexplored. 

In this paper, we systematically compare the performance between two algorithm modes, FedSGD and FedAvg that correspond to aggregating gradients and models, respectively. Our results across various task scenarios indicate these two modes exhibit a substantial performance gap. Specifically, FedSGD achieves higher accuracy and faster convergence but experiences more severe fluctuations in accuracy, whereas FedAvg excels in handling straggler issues but converges slower with reduced accuracy.


%Federated learning is valued research for its high-performance computing in distributed environments while safeguarding data privacy. In addressing the issue of resource heterogeneous, researchers have proposed a semi-asynchronous federated learning architecture, which enables participants to autonomously train local models and update. However, the performance gap between aggregating models and gradients in SAFL remains unexplored. 

%In this paper, we conducted a comparative analysis between aggregating models and gradients. Results across various task scenarios indicate that these two aggregation targets exhibit substantial performance gap, where aggregating gradients, i.e. \sgd, achieves higher accuracy and faster convergence but fluctuates in accuracy, whereas aggregating models, i.e. \avg, excels in handling straggler issues but converges slower with reduced accuracy. To bridge the performance gap between different aggregation targets, we also propose an algorithm \tool deploying a few-shot datasets on the server to supervise the aggregation process. Experimental results show improved accuracy and convergence for both methods.


\end{abstract}

\begin{IEEEkeywords}
Federated Learning, Semi-Asynchronous Distribution Learning, Performance Gap, Prediction Accuracy, Convergence Stability
\end{IEEEkeywords}

==> contents/exper_ret.tex <==
\section{Experimental Results and Discussion}
In this section, we will first introduce several measurement criteria for evaluating experimental results. Subsequently, we will present our experimental results on different datasets and provide some analysis of the outcomes.

\subsection{Measurement Criteria}
Our primary approach involves conducting experimental evaluations of federated learning across diverse scenarios and aggregation targets, focusing on assessing key metrics such as accuracy, loss, resource utilization, time consumption, convergence and so on.

\subsubsection{Accuracy and Loss}
We evaluate the accuracy and loss of the global model on the test dataset following each global aggregation, documenting the training epochs and the total training time. In the case of image datasets, we utilize the test dataset split directly provided by PyTorch. For text datasets, we adopt a uniform sampling approach, selecting 20\% of the data as the test dataset and ensure that these data points are distinct from those included in the training set, maintaining the integrity of the evaluation process. Meanwhile, we denote NaN as -1 in loss.

\subsubsection{Resource utilization}
We will evaluate federated learning resource consumption in different scenarios from three perspectives: memory usage, training duration, and channel transmission load. These three metrics can be directly measured during the training process and are relatively easy to obtain for comparison.

\subsubsection{Accumulated staleness}
First, we will provide a definition for staleness in semi-asynchronous federated learning: for a client $C_i$, it starts its local train with the newest global model $w_g^{t_0}$ and finish its local train when getting the model $w_{i,E}^{t_0}$. If the gradient or the model it sends to the server is used to aggregate the global model under the $t$-th global epoch, then we say that this data uploaded from $C_i$ has a staleness as $\tau_s^t$ under the $t$-th global epoch, where:
\begin{equation}
    \tau_s^t = t - t_0 - 1
\end{equation}

It's obvious that $\tau_s^t \geq 0$ and when a participant can complete local training rapidly enough, meaning that it uploads data for aggregation in the $t$-th round immediately after training its local model with the $(t-1)$-th round's model, the staleness of data is considered to be $0$ since $\tau_s^t = t - (t-1) -1 = 0$.

Based on the definition of staleness, we calculate the cumulative staleness of the clients participating in each global aggregation as:
\begin{equation}
    \tau^t = \sum_{s \in \mathcal{S}} \tau_s^t
\end{equation}

We believe that such cumulative staleness can reflect the overall impact of stragglers on the aggregation process in a given global epoch. A higher cumulative staleness indicates a greater degree of straggling among participants and a higher likelihood of negative effects on model aggregation.

\begin{figure*}[!tp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2in]{pic/ret/resnet18_cifar10/HD/acc/0.1.png}%
\label{fig_acc_resnet_cifar10_HD_01}}
\hspace{1mm}
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2in]{pic/ret/resnet18_cifar10/HD/acc/0.5.png}%
\label{fig_acc_resnet_cifar10_HD_05}}  
\hspace{1mm}
\subfloat[$\alpha = 1$]{\includegraphics[width=2in]{pic/ret/resnet18_cifar10/HD/acc/1.png}%
\label{fig_acc_resnet_cifar10_HD_1}}
\caption{Global accuracy of ResNet-18 model under Cifar-10 dataset with Hetero Dirichlet distribution}
\label{fig_acc_resnet_cifar10_HD}
\end{figure*}

\begin{figure*}[!tp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar10/HD/loss/0.1.png}%
\label{fig_loss_resnet_cifar10_HD_01}}
\hspace{1mm}
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar10/HD/loss/0.5.png}%
\label{fig_loss_resnet_cifar10_HD_05}}  
\hspace{1mm}
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar10/HD/loss/1.png}%
\label{fig_loss_resnet_cifar10_HD_1}}
\caption{Global loss of resnet-18 model under cifar-10 dataset with hetero Dirichlet distribution}
\label{fig_loss_resnet_cifar10_HD}
\end{figure*}

\begin{figure*}[!tp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/acc/0.1.png}%
\label{fig_acc_vgg16_cifar10_HD_01}}
\hspace{-5mm}
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/acc/0.5.png}%
\label{fig_acc_vgg16_cifar10_HD_05}}  
\hspace{-5mm}
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/acc/1.png}%
\label{fig_acc_vgg16_cifar10_HD_1}}
\caption{Global accuracy of vgg16 model under cifar-10 dataset with hetero Dirichlet distribution}
\label{fig_acc_vgg16_cifar10_HD}
\end{figure*}

\begin{figure*}[!tp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/loss/0.1.png}%
\label{fig_loss_vgg16_cifar10_HD_01}}
\hspace{-5mm}
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/loss/0.5.png}%
\label{fig_loss_vgg16_cifar10_HD_05}}  
\hspace{-5mm}
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/loss/1.png}%
\label{fig_loss_vgg16_cifar10_HD_1}}
\caption{Global accuracy of vgg16 model under cifar-10 dataset with hetero Dirichlet distribution}
\label{fig_loss_vgg16_cifar10_HD}
\end{figure*}

\begin{figure*}[!htp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/acc/0.1.png}%
\label{fig_acc_resnet_cifar100_HD_01}}
\hspace{-5mm}
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/acc/0.5.png}%
\label{fig_acc_resnet_cifar100_HD_05}}  
\hspace{-5mm}
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/acc/1.png}%
\label{fig_acc_resnet_cifar100_HD_1}}
\caption{Global accuracy of resnet-18 model under cifar-100 dataset with hetero Dirichlet distribution}
\label{fig_acc_resnet_cifar100_HD}
\end{figure*}

\begin{figure*}[!htp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/loss/0.1.png}%
\label{fig_loss_resnet_cifar100_HD_01}}
\hspace{-5mm}
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/loss/0.5.png}%
\label{fig_loss_resnet_cifar100_HD_05}}  
\hspace{-5mm}
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/loss/1.png}%
\label{fig_loss_resnet_cifar100_HD_1}}
\caption{Global loss of resnet-18 model under cifar-100 dataset with hetero Dirichlet distribution}
\label{fig_loss_resnet_cifar100_HD}
\end{figure*}

\subsubsection{Convergence}
Although accuracy and loss function curves over training epochs provide a qualitative analysis of training convergence, we provide additional quantitative indicators to better illustrate convergence including 
the epochs required to achieve the target accuracy $Acc_t$ for the first time, denoted by $T_f$, and the epochs after which the model remains stable above the target accuracy $Acc_t$, denoted by $T_s$. Additionally, we also counted the number of instances where the training process experienced severe oscillations, denoted by $O_{ots}$ where $ots$ is an oscillation threshold. We define severe oscillations as follows: the accuracy in the current round is lower than the accuracy in the previous round by a certain threshold, then it is considered to have experienced a severe oscillation.

In our definition, determining the target accuracy $Acc_t$ and oscillation threshold $ots$ is a crucial aspect. The selection of these values often varies across different experimental scenarios. In our study, we empirically chose these values based on the obtained experimental data.

\subsection{Experimental Results}
Then, we will demonstrate the results of different aggregation targets in various experimental scenarios. The results show that there is a significant gap. Due to space constraints, we only present part of the experimental results to illustrate our conclusion. More experimental results will be shown in the appendix.

\subsubsection{Loss and acc}

Fig.~\ref{fig_acc_resnet_cifar10_HD} and Fig.~\ref{fig_loss_resnet_cifar10_HD} shows the lobal accuracy and global loss on Resnet-18 under under cifar-10 dataset with hetero Dirichlet distribution. And the Fig.~\ref{fig_acc_vgg16_cifar10_HD} and Fig.~\ref{fig_loss_vgg16_cifar10_HD} shows the lobal accuracy and global loss on VGG16 under under cifar-10 dataset with hetero Dirichlet distribution. The figures Fig.~\ref{fig_acc_resnet_cifar10_HD} and Fig.~\ref{fig_acc_vgg16_cifar10_HD} implement that aggregating gradient can achieve higher accuracy than aggregating model weights in semi-asynchronous federated learning and the figures Fig.~\ref{fig_loss_resnet_cifar10_HD} and Fig.~\ref{fig_loss_vgg16_cifar10_HD} implement that aggregating gradient will result in the loss becoming NaN. Aggregating model weights, on the other hand, won't result in this. Meanwhile, as the non-iid degree of data distribution increases, NaN occurs more frequently in loss.

Fig.~\ref{fig_acc_resnet_cifar100_HD} and Fig.~\ref{fig_loss_resnet_cifar100_HD} shows the lobal accuracy and global loss on Resnet-18 under under cifar-100 dataset with Hetero Dirichlet distribution. Fig.~\ref{fig_acc_resnet18_cifar10_Shards} and Fig.~\ref{fig_loss_resnet18_cifar10_Shards} shows the lobal accuracy and global loss on Resnet-18 under under cifar-10 dataset with Shards distribution. These results implement that under different dataset and different data distributions, aggregating gradients show the same impact on the global model.

\begin{figure}[!tp]
\centering
\subfloat[$\alpha = 5$]{\includegraphics[width=1.7in]{pic/ret/resnet18_cifar10/shards/acc/5.png}%
\label{fig_acc_resnet18_cifar10_Shards_5}}
\hfil
\subfloat[$\alpha = 10$]{\includegraphics[width=1.7in]{pic/ret/resnet18_cifar10/shards/acc/5.png}%
\label{fig_acc_resnet18_cifar10_Shards_10}}
\caption{Global accuracy of resnet-18 model under cifar-10 dataset with Shards distribution}
\label{fig_acc_resnet18_cifar10_Shards}
\end{figure}

\begin{figure}[!tp]
\centering
\subfloat[$\alpha = 5$]{\includegraphics[width=1.7in]{pic/ret/resnet18_cifar10/shards/loss/5.png}%
\label{fig_loss_resnet18_cifar10_Shards_5}}
\hfil
\subfloat[$\alpha = 10$]{\includegraphics[width=1.7in]{pic/ret/resnet18_cifar10/shards/loss/5.png}%
\label{fig_loss_resnet18_cifar10_Shards_10}}
\caption{Global loss of resnet-18 model under cifar-10 dataset with Shards distribution}
\label{fig_loss_resnet18_cifar10_Shards}
\end{figure}

Under LSTM model and Shakespeare dataset, we conducted experiments on a text prediction task which show the same results with computer vision tasks. Aggregating gradients can reached the accuracy of synchronous federated learning while aggregating model weights have a relatively quite low accuracy. Moreover, there still exists NaN when using gradients to aggregate global model.
\begin{figure}[!tp]
\centering
\subfloat[Client=$100$]{\includegraphics[width=1.7in]{pic/ret/LSTM/100/acc/0.8.png}%
\label{fig_acc_LSTM_100}}
\hfil
\subfloat[Client=$300$]{\includegraphics[width=1.7in]{pic/ret/LSTM/300/acc/0.8.png}%
\label{fig_acc_LSTM_300}}
\caption{Global accuracy of LSTM model under Shakespeare dataset}
\label{fig_LSTM_acc}
\end{figure}

\begin{figure}[!tp]
\centering
\subfloat[Client=$100$]{\includegraphics[width=1.7in]{pic/ret/LSTM/100/loss/0.8.png}%
\label{fig_loss_LSTM_100}}
\hfil
\subfloat[Client=$300$]{\includegraphics[width=1.7in]{pic/ret/LSTM/300/loss/0.8.png}%
\label{fig_loss_LSTM_300}}
\caption{Global loss of LSTM model under Shakespeare dataset}
\label{fig_LSTM_loss}
\end{figure}
\subsubsection{Resource Consumption}
We compiled resource consumption and show this in Table. 

\begin{table*}[!htp]
    \caption{Resource Consumption under different environments in semi-asynchronous federated learning}
    \centering
    \begin{threeparttable}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
       Model & Dataset & Distribution &Scheme & Memory Usage $/GB$ & Training duration $/s$ & Channel Transmission Load $/MB$\\
    \hline
         \multirow{2}{*}{ResNET-18} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Hetero Dirichlet} &FedAvg & 34 & 61832 & 198294\\\cline{4-7} 
          &  & &FedSGD & 34 & 61529 & 171803\\\hline
          \multirow{2}{*}{ResNET-18} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Shards} &FedAvg &  34 & 35371 & 198294\\\cline{4-7} 
          &  & &FedSGD & 33 & 33326 & 171803\\\hline
          \multirow{2}{*}{ResNET-18} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Unbalance} &FedAvg & 30 & 45323 & 198294\\\cline{4-7} 
          &  & &FedSGD & 29 & 37679 & 171803\\\hline
          \multirow{2}{*}{ResNET-18} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Hetero Dirichlet} &FedAvg & 58 & 82704 & 198294\\\cline{4-7} 
          &  & &FedSGD & 55 & 78802 & 171803\\\hline
          \multirow{2}{*}{ResNET-18} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Shards} &FedAvg &  57 & 82062 & 198294\\\cline{4-7} 
          &  & &FedSGD & 56 & 51396 & 171803\\\hline
          \multirow{2}{*}{ResNET-18} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Unbalance} &FedAvg & 50 & 40055 & 198294\\\cline{4-7} 
          &  & &FedSGD & 48 & 34724 & 171803\\\hline
          \multirow{2}{*}{VGG-16} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Hetero Dirichlet} &FedAvg & 45 & 87265 & 515067\\\cline{4-7} 
          &  & &FedSGD & 43 & 86979 & 512896\\\hline
          \multirow{2}{*}{VGG-16} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Shards} &FedAvg &  45 & 84541 & 515067\\\cline{4-7} 
          &  & &FedSGD & 44 & 84516 & 512896\\\hline
          \multirow{2}{*}{VGG-16} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Unbalance} &FedAvg & 40 & 68426 & 515067\\\cline{4-7} 
          &  & &FedSGD & 40 & 62767 & 512896\\\hline
          \multirow{2}{*}{VGG-16} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Hetero Dirichlet} &FedAvg & 68 & 61295 & 515067\\\cline{4-7} 
          &  & &FedSGD & 66 & 58736 & 512896\\\hline
          \multirow{2}{*}{VGG-16} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Shards} &FedAvg &  68 & 62203 & 515067\\\cline{4-7} 
          &  & &FedSGD & 66 & 60965 & 512896\\\hline
          \multirow{2}{*}{VGG-16} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Unbalance} &FedAvg & 65 & 45286 & 515067\\\cline{4-7} 
          &  & &FedSGD & 64 & 42030 & 512896\\\hline
          \multirow{2}{*}{CNN} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Hetero Dirichlet} &FedAvg & 22 & 4291 & 4374.72 \\\cline{4-7} 
          &  & &FedSGD & 20 & 4261 & 4173.72\\\hline
          \multirow{2}{*}{CNN} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Shards} &FedAvg & 22 & 4859.6 & 4374.72\\\cline{4-7} 
          &   & &FedSGD & 21 & 4819.3 & 4173.72\\\hline
          \multirow{2}{*}{CNN} & \multirow{2}{*}{Cifar-10} & \multirow{2}{*}{Unbalance} &FedAvg &  16 & 3181 & 4374.72\\\cline{4-7} 
          &  & &FedSGD & 15 & 2209.5 & 4173.72\\\hline
          \multirow{2}{*}{CNN} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Hetero Dirichlet} &FedAvg & 44 & 29173 & 4374.72\\\cline{4-7} 
          &  & &FedSGD & 42 & 28434 & 4173.72\\\hline
          \multirow{2}{*}{CNN} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Shards} &FedAvg & 42 & 27018 & 4374.72\\\cline{4-7} 
          &  & &FedSGD & 41 & 25450 & 4173.72\\\hline
          \multirow{2}{*}{CNN} & \multirow{2}{*}{FEMNIST} & \multirow{2}{*}{Unbalance} &FedAvg &  35 & 14815 & 4374.72\\\cline{4-7} 
          &  & &FedSGD & 33 & 12326 & 4173.72\\\hline
          \multirow{2}{*}{LSTM} & \multirow{2}{*}{Shakespeare} & \multirow{2}{*}{client=100} &FedAvg & 20 & 43244 & 3472\\\cline{4-7} 
          &  & &FedSGD & 19 & 43216 & 3434\\\hline
          \multirow{2}{*}{LSTM} & \multirow{2}{*}{Shakespeare} & \multirow{2}{*}{client=300} &FedAvg & 63 & 87655 & 3472\\\cline{4-7} 
          &  & &FedSGD & 60 & 87583 & 3434\\
    \hline
    \end{tabular}
     \begin{tablenotes}
        \footnotesize
        \item[*] For the Dirichlet distribution, we choose parameters as $\alpha=0.5$; For Shards distribution, we choose parameters as $\alpha = 5$; For Unbalance Dirichlet distribution, we choose parameters as $\alpha=0.5$
      \end{tablenotes}
\end{threeparttable}
\end{table*}


\subsubsection{convergence}
To evaluate convergence, we first show the severe oscillations in different enviroments.
\begin{figure*}[!htp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar10/HD/ots/0.1.png}%
\label{fig_resnet18_cifar10_HD_ots_01}}
\hfil
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar10/HD/ots/0.5.png}%
\label{fig_resnet18_cifar10_HD_ots_05}}
\hfil
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar10/HD/ots/1.png}%
\label{fig_resnet18_cifar10_HD_ots_1}}                
\caption{severe oscillations of resnet-18 model under cifar-10 dataset with Hetero Dirichlet distribution}
\label{fig_resnet18_cifar10_HD_ots}
\end{figure*}

\begin{figure*}[!htp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/ots/0.1.png}%
\label{fig_resnet18_cifar100_HD_ots_01}}
\hfil
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/ots/0.5.png}%
\label{fig_resnet18_cifar100_HD_ots_05}}
\hfil
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/resnet18_cifar100/HD/ots/1.png}%
\label{fig_resnet18_cifar100_HD_ots_1}}                
\caption{severe oscillations of resnet-18 model under cifar-100 dataset with Hetero Dirichlet distribution}
\label{fig_resnet18_cifar100_HD_ots}
\end{figure*}

\begin{figure*}[!htp]
\centering
\subfloat[$\alpha = 0.1$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/ots/0.1.png}%
\label{fig_vgg16_cifar10_HD_ots_01}}
\hfil
\subfloat[$\alpha = 0.5$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/ots/0.5.png}%
\label{fig_vgg16_cifar10_HD_ots_05}}
\hfil
\subfloat[$\alpha = 1$]{\includegraphics[width=2.3in]{pic/ret/vgg16_cifar10/HD/ots/1.png}%
\label{fig_vgg16_cifar10_HD_ots_1}}                
\caption{severe oscillations of vgg16 model under cifar-10 dataset with Hetero Dirichlet distribution}
\label{fig_vgg16_cifar10_HD_ots}
\end{figure*}

\begin{table}[!htp]
    \caption{Convergence situation by ResNET-18 model and CIFAR-10 dataset}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Distribution& $\alpha$ & Scheme &Threshold & tf & ts \\
    \hline
          \multirow{6}{*}{Hetero  Dirichlet} &   \multirow{2}{*}{0.1} & Avg & 50\% & 208 & 399\\\cline{3-6}
          &  & SGD & 50\% & 86 & 324 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 60\% & 195 & 341\\\cline{3-6} 
          &  & SGD & 60\% & 82 &349 \\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 60\% & 107 &  119\\\cline{3-6} 
          &  & SGD & 60\% & 57 &282 \\\hline

          \multirow{6}{*}{Unbalance  Dirichlet}  & \multirow{2}{*}{0.1} & Avg & 50\% & 331 & 380\\\cline{3-6}
          &  & SGD & 50\% & 132 & 201 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 50\% & 358 & 399 \\\cline{3-6} 
          &  & SGD & 60\% & 254 & 397\\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 60\% & 262 & 320 \\\cline{3-6} 
          &  & SGD & 60\% & 171 & 242\\\hline
          
          \multirow{4}{*}{Shards}   & \multirow{2}{*}{5} & Avg & 60\% & 129 & 339\\\cline{3-6}
          &  & SGD & 60\% & 84 & 398 \\\cline{2-6} 
          &  \multirow{2}{*}{10} & Avg & 70\%& 218& 289\\\cline{3-6}
          &  & SGD & 70\% & 99 & 229\\
            
    \hline
    \end{tabular}
\end{table}

\begin{table}[!htp]
    \caption{Convergence situation by ResNET-18 model and CIFAR-100 dataset}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Distribution& $\alpha$ & Scheme &Threshold & tf & ts \\
    \hline
          \multirow{6}{*}{Hetero  Dirichlet} &   \multirow{2}{*}{0.1} & Avg & 40\% & 369 & 400\\\cline{3-6}
          &  & SGD & 50\% & 223 & 329\\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 40\% & 225 & 293 \\\cline{3-6} 
          &  & SGD & 55\% &202 & 328 \\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 40\% & 246 & 329 \\\cline{3-6} 
          &  & SGD & 55\% & 184& 328 \\\hline

          \multirow{6}{*}{Unbalance  Dirichlet}  & \multirow{2}{*}{0.1} & Avg & 10\% & 308& 393\\\cline{3-6}
          &  & SGD & 10\% & 92 & 167 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 10\% & 76& 103\\\cline{3-6} 
          &  & SGD & 10\% & 70 & 72 \\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 10\% & 311 & 398 \\\cline{3-6} 
          &  & SGD & 10\% & 182 & 193 \\\hline
          
          \multirow{4}{*}{Shards}   & \multirow{2}{*}{5} & Avg & 15\% & 239 & 342\\\cline{3-6}
          &  & SGD & 15\% & 84 &346 \\\cline{2-6} 
          &  \multirow{2}{*}{10} & Avg & 250\% & 232 & 286 \\\cline{3-6}
          &  & SGD & 45\% & 246 & 335\\
            
    \hline
    \end{tabular}
\end{table}

\begin{table}[!htp]
    \caption{Convergence situation by ResNET-18 model and FEMNIST dataset}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Distribution& $\alpha$ & Scheme &Threshold & tf & ts \\
    \hline
          \multirow{6}{*}{Hetero  Dirichlet} &   \multirow{2}{*}{0.1} & Avg & 75\% & 28 & 142 \\\cline{3-6}
          &  & SGD & 75\% & 16 & 197 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 75\% & 10 & 30 \\\cline{3-6} 
          &  & SGD & 75\% & 9 & 44 \\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 80\% & 16 & 33 \\\cline{3-6} 
          &  & SGD & 80\% & 14 &149 \\\hline

          \multirow{6}{*}{Unbalance  Dirichlet}  & \multirow{2}{*}{0.1} & Avg & 70\% & 101 & 199\\\cline{3-6}
          &  & SGD & 70\% & 22 & 191 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 70\% & 14 & 33\\\cline{3-6} 
          &  & SGD & 70\% & 10 & 44\\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 75\% & 40 & 82 \\\cline{3-6} 
          &  & SGD & 75\% & 23 & 105 \\\hline
          
          \multirow{4}{*}{Shards}   & \multirow{2}{*}{5} & Avg & 70\% & 192 & 198 \\\cline{3-6}
          &  & SGD & 70\% & 60 & 200 \\\cline{2-6} 
          &  \multirow{2}{*}{10} & Avg & 75\%& 94& 191\\\cline{3-6}
          &  & SGD & 75\% & 40&195\\
            
    \hline
    \end{tabular}
\end{table}

\begin{table}[!htp]
    \caption{Convergence situation by VGG-16 model and CIFAR-10 dataset}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Distribution& $\alpha$ & Scheme &Threshold & tf & ts \\
    \hline
          \multirow{6}{*}{Hetero  Dirichlet} &   \multirow{2}{*}{0.1} & Avg & 25\% & 149 & 390\\\cline{3-6}
          &  & SGD & 25\% & 53 & 393 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 55\% & 348 & 395 \\\cline{3-6} 
          &  & SGD & 55\% & 181 & 393 \\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 65\% & 395 & 397 \\\cline{3-6} 
          &  & SGD & 65\% & 167 & 369 \\\hline

          \multirow{6}{*}{Unbalance  Dirichlet}  & \multirow{2}{*}{0.1} & Avg & 25\% & 255 & 389 \\\cline{3-6}
          &  & SGD & 25\% & 136 & 346 \\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 25\% & 101 & 353 \\\cline{3-6} 
          &  & SGD & 25\% & 47 & 300 \\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 30\% & 68 & 154 \\\cline{3-6} 
          &  & SGD & 30\% & 35 & 199 \\\hline
          
          \multirow{4}{*}{Shards}   & \multirow{2}{*}{5} & Avg & 30\% & 111 & 365\\\cline{3-6}
          &  & SGD & 30\% & 74 & 398\\\cline{2-6} 
          &  \multirow{2}{*}{10} & Avg & 30\% & 103 & 274\\\cline{3-6}
          &  & SGD &30\% & 57 & 349\\
            
    \hline
    \end{tabular}
\end{table}

\begin{table}[!htp]
    \caption{Convergence situation by CNN model and CIFAR-10 dataset}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
         Distribution& $\alpha$ & Scheme &Threshold & tf & ts \\
    \hline
          \multirow{6}{*}{Hetero  Dirichlet} &   \multirow{2}{*}{0.1} & Avg & 40\%& 168& 376\\\cline{3-6}
          &  & SGD & 60\% & 251 & 377\\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 50\% & 175& 229\\\cline{3-6} 
          &  & SGD & 60\% & 167 & 328\\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 50\%& 229 & 262 \\\cline{3-6} 
          &  & SGD & 65\%& 179 & 302 \\\hline

          \multirow{6}{*}{Unbalance  Dirichlet}  & \multirow{2}{*}{0.1} & Avg & 20\% & 288 & 363\\\cline{3-6}
          &  & SGD & 30\% & 215 & 354\\\cline{2-6} 
          &  \multirow{2}{*}{0.5} & Avg & 40\% & 215 & 227 \\\cline{3-6} 
          &  & SGD & 40\% & 77 & 166\\\cline{2-6} 
          &  \multirow{2}{*}{1} & Avg & 45\% & 360 & 391 \\\cline{3-6} 
          &  & SGD & 45\% & 158 & 328\\\hline
          
          \multirow{4}{*}{Shards}   & \multirow{2}{*}{5} & Avg & 50\% & 317 & 399\\\cline{3-6}
          &  & SGD & 50\% & 137 & 400 \\\cline{2-6} 
          &  \multirow{2}{*}{10} & Avg & 50\% & 247 & 358 \\\cline{3-6}
          &  & SGD & 50\% & 109 & 229\\
            
    \hline
    \end{tabular}
\end{table}
\subsection{Cause Analysis}
From the above subsection, we know there exist significant differences between gradient aggregation and model weight aggregation. In this section, we will give some quantity analysis to discuss the difference.

\subsubsection{Directional gradients}
It's a clear conclusion that gradients are vectors with direction and model weights are scalars without direction and directional gradients is a reasonable explanation to the difference of gradient aggregation between SFL and SAFL. Since the gradients in set $\mathcal{AC}$ have no staleness in synchronous federated learning, every gradients have less deviation from the most recent global epoch. However, server has challenge to control the aggregation sequence in semi-asynchronous federated learning, the set waiting to aggregation $\mathcal{S}$ will have different gradients with different staleness and  there is a high probability of the existence of some gradients with high staleness resulting in high deviation from the unbiased direction. These deviation may cause the aggregated gradient be 0 and this is the reason for gradient vanishing to be NaN. A intuitive illustration is visually represented in Fig.~\ref{fig_gradient}.

\begin{figure}[!tp]
\centering
\subfloat[]{\includegraphics[width=1in]{pic/gradient/SFL_normal.png}%
\label{fig_SFL_gradient}}
\hfil
\subfloat[]{\includegraphics[width=1in]{pic/gradient/SAFL_normal.png}%
\label{fig_SAFL_gradient}}
\hfil
\subfloat[]{\includegraphics[width=1in]{pic/gradient/SAFL_NAN.png}%
\label{fig_SAFL_gradient_NAN}}                
\caption{Directional Gradient Aggregation (a) in SFL; (b) in SAFL, a normal case; (c) in SAFL, a special case}
\label{fig_gradient}
\end{figure}

The following experiment results also provide evidence for this reason. In Zhou et al.\cite{zhou2022towards}'s research, they propose that estimated gradient after clipping the gradients is benefit for gradient aggregation. We use clip scheme in resnet-18 model and Hetero-Dirichlet distribution on cifar-10 dataset to control the bound of the gradients. Fig.~ shows the results.




\subsubsection{Aggregation effectiveness}
The difference of aggregation effectiveness is also a factor causing the difference between aggregation gradient and aggregation model weight. From the Equ.~\ref{equ:fedsgd_update} and Equ.~\ref{equ:fedavg_update}, we can find that the global aggregation model for one global epoch is determined by the data (model weights or gradients) uploaded by the clients. It's obvious that each uploaded model is effective on its dataset. Regardless of how outdated the model may be, the aggregated model after aggregation remains effective, but the model will exhibiting a greater level of bias\cite{wang2019adaptive}. However, maintaining this effectiveness can lead to the aggregation of models being more prone to falling into the local optimum.  From another perspective, as can be seen from Fig.~\ref{fig_gradient}, using gradients to aggregate global model will break the effectiveness frequenly. This means that gradient aggregation has a larger step size in optimization problems and has high possibility to find the global optimum.

==> contents/exper_steup.tex <==
\section{Experimental Set-up}
In this section, we will introduce the data and models used for comparative experimental analysis.

\subsection{Data Sets}
We will first introduce the datasets used in our experiments, including three types of image data and one type of language text data.

\subsubsection{CIFAR-10}
CIFAR-10 is a widely used benchmark dataset for image classification tasks in machine learning. It consists of $10$ labels, with each class containing $6,000$ images with a size of $32\times32$ and in RGB format.
\subsubsection{CIFAR-100}
CIFAR-100 is more complex compared to CIFAR-10, with a total of 100 categories. Each category comprises $600$ images sized $32\times32$ and in $RGB$ format.
\subsubsection{FEMNIST}
FEMNIST(Federated Extended MNIST) is an improved dataset derived from the EMNIST dataset, specifically designed for the characteristics of federated learning scenarios. It is utilized for handwritten character recognition tasks. This dataset comprises $62$ classes of handwritten character data, with each image being a gray-scale $28\times28$ image.
\subsubsection{Shakespeare}
This dataset is a text dataset used for natural language processing tasks. It compiles all literary works of William Shakespeare. We embedded 80 characters, including 26 uppercase English characters, 26 lowercase English characters, 10 numeric characters, and 18 special characters, to 80 labels. Next, we divided Shakespeare's works into text data, using a sliding window with a length of 80 and a step size of 1. What's more, we divided the dataset into training and testing sets with a ratio of 80\% and 20\% in our experiment. The specific details of data partitioning will be discussed in the next section.

\subsection{Data Distributions}
In real-world scenarios, federated learning may encounter diverse data distribution situations. This section introduces the data distribution scenarios employed in this paper.

Firstly, we will introduce the distribution of image data, encompassing one that is independently and identically distributed (IID) and three that are non-IID.

\subsubsection{Balanced Independently and Identically Distribution}
In this IID scenario, each participant possesses data covering all labels with an equal amount of data. Simultaneously, the data distributions among clients are entirely identical. Under these conditions, federated learning is nearly indistinguishable from centralized learning.

\subsubsection{Shards Distribution}
Each participant holds an equal quantity of data but only covers specific labels. In extreme cases, the data distribution among participants is entirely distinct. For example, two participants $\mathcal{C} = \{C_1, C_2\}$ are preparing to collaborate for federated learning. However, $C_1$ has 500 data points with label $a$, and $C_2$ has 500 data points with label $b$. Although both of them have an equal quantity of data, neither possesses data corresponding to all labels, and their data distributions are entirely different.
\begin{figure}[!htp]
\centering
\subfloat[Shards = 5]{\includegraphics[width=1.7in]{pic/distribution/Shards/5.png}%
\label{fig_Distribution_Shards5}}
\hfil
\subfloat[Shards = 10]{\includegraphics[width=1.7in]{pic/distribution/Shards/10.png}%
\label{fig_Distribution_Shards10}}
\caption{Data Distribution under Shards Distribution.}
\label{fig_Distribution_Shards}
\end{figure}
\subsubsection{Unbalanced Dirichlet Distribution}
Each participant possesses data for all labels, and the data distribution is identical among participants.  However, there are variations in the quantity of data each participant possesses. The data distribution for each participant follows a Dirichlet distribution $Dir(\alpha)$ as:
\begin{equation}
    D(p|\alpha) = \frac{\Gamma(\sum_{i=1}^N \alpha_i)}{\Pi_{i=1}^N\Gamma(\alpha_i)}\Pi_{i=1}^Np_i^{\alpha_i-1}
\end{equation}

The distribution of data quantity follows a log-normal distribution $Log-N(0,\sigma^2)$ as:
\begin{equation}
    f(x) = \frac{1}{x\sigma\sqrt{2\pi}}exp(-\frac{(\ln(x))^2}{2\sigma^2})
\end{equation}

\begin{figure}[!htp]
\centering
\subfloat[$\sigma^2 = 1$]{\includegraphics[width=1.7in]{pic/distribution/UD/1Client_distribution.png}%
\label{fig_Distribution_UD1_amount}}
\hfil
\subfloat[$\sigma^2 = 0.1$]{\includegraphics[width=1.7in]{pic/distribution/UD/0.1Client_distribution.png}%
\label{fig_Distribution_UD_01_amount}}
\hfil
\subfloat[$\sigma^2 = 1$]{\includegraphics[width=1.7in]{pic/distribution/UD/1.png}%
\label{fig_Distribution_UD1}}
\hfil
\subfloat[$\sigma^2 = 0.1$]{\includegraphics[width=1.7in]{pic/distribution/UD/0.1.png}%
\label{fig_Distribution_UD_01}}
\caption{Data Distribution under Unbalanced Dirichlet Distribution. (a)(b) Distribution of the amount of data; (c)(d) Distribution of the class of each client }
\label{fig_Distribution_UD}
\end{figure}

\subsubsection{Hetero Dirichlet Distribution}
This type of distribution is more commonly observed in real-world scenarios. Each participant possesses data corresponding to a subset of labels, with unequal data quantities and distinct data distributions among participants. The data for each participant forms a Dirichlet distribution based on categories as $D_k(\alpha)$.
\begin{equation}
    D(p_k|\alpha) = \frac{\Gamma(\sum_{i=1}^N \alpha_i)}{\Pi_{i=1}^N\Gamma(\alpha_i)}\Pi_{i=1}^Np_{k,i}^{\alpha_i-1}
\end{equation}

\begin{figure}[!htp]
\centering
\subfloat[$\alpha = 1$]{\includegraphics[width=1.7in]{pic/distribution/HD/1Client_distribution.png}%
\label{fig_Distribution_HD1_amount}}
\hfil
\subfloat[$\alpha = 0.3$]{\includegraphics[width=1.7in]{pic/distribution/HD/0.3Client_distribution.png}%
\label{fig_Distribution_HD_03_amount}}
\hfil
\subfloat[$\alpha = 1$]{\includegraphics[width=1.7in]{pic/distribution/HD/1.png}%
\label{fig_Distribution_HD1}}                
\hfil
\subfloat[$\alpha = 0.3$]{\includegraphics[width=1.7in]{pic/distribution/HD/0.3.png}%
\label{fig_Distribution_HD_03}}
\caption{Data Distribution under Unbalanced Dirichlet Distribution. (a)(b) Distribution of the amount of data; (c)(d) Distribution of the class of each client }
\label{fig_Distribution_HD}
\end{figure}

Next, we will introduce the distribution of text data, where we followed the benchmark approach and partitioned the text data.

\subsubsection{IID text data}
The definition of independently and identically distributed data in the text dataset is somewhat ambiguous. We consider the data to be IID when all participants uniformly sample without distinguishing character roles, meaning each participant's data is independently and identically distributed to others.

\subsubsection{non-IID text data}
On the other hand, we consider the dialogues of different characters in different scripts to be non-IID. As long as each participant is assigned data generated from dialogue lines of different characters in different scripts, the data distribution among these participants is non-IID. Below is an example of  participant's datasets in a non-IID scenario.
\begin{table}[!htp]
    \caption{An example of non-IID Shakespeare Data}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
       User  & Scripts & Role & Amount \\
    \hline
         1 & ALLS WELL THAT ENDS WELL & BERTRAM & 10538 \\\hline
         2 & ALLS WELL THAT ENDS WELL & CLOWN & 8391 \\\hline
         3 & AS YOU LIKE IT & AMIENS & 629 \\\hline
         4 & CYMBELINE & QUEEN & 6612 \\\hline
         5 & \makecell[c]{SECOND PART OF\\ KING HENRY IV} & PRINCE & 8820 \\\hline
         6 & \makecell[c]{TWELFTH NIGHT;\\ OR, WHAT YOU WILL }& CLOWN & 10985 \\\hline
         7 & KING HENRY THE EIGHTH & DENNY & 39 \\
    \hline
    \end{tabular}
    
\end{table}

\subsection{Models}
We utilize the following three models to accomplish the image classification task.
\subsubsection{CNN}
CNN (Convolutional Neural Network) is a classic deep learning neural network model. The CNN used in this paper consists of three convolutional layers using 3x3 kernels with a stride of 1., one max-pooling layer, and two fully connected layers, with the ReLU activation function applied.

\subsubsection{Resnet-18}
ResNet is a family of residual networks that introduced the concept of residual blocks. The residual blocks use skip connection to addresses the issues of vanishing and exploding gradients in deep neural networks and make information smoothly transmit. ResNet-18 is one of the smaller structures in the ResNet family, comprising 18 layers with four residual blocks. Each residual block consists of two convolutional layers using 3x3 kernels with a stride of 1.
\subsubsection{VGG-16}
VGG (Visual Geometry Group) is a specific architecture of Convolutional Neural Network (CNN) designed for computer vision tasks. The model adopted in this paper is VGG-16, which consists of 13 convolutional layers and 3 fully connected layers, with a relatively large parameter scale.


On the other hand, we employ the LSTM model to fulfill text prediction tasks.
\subsubsection{LSTM}
LSTM (Long Short-Term Memory) is a special type of recurrent neural network (RNN) designed for handling and learning sequential data. Compared to traditional RNNs, LSTM is designed to address the issues of vanishing and exploding gradients on long sequential data. It excels in capturing and processing long-term dependencies, making it particularly effective for natural language processing tasks. In our experiments, the simplest LSTM model was employed, consisting of one embedding layer, one LSTM layer, and one fully connected layer.

==> contents/formulation.tex <==
\section{Problem Formulation}
In this section, we first introduce the basic FL notations, along with two representative algorithms FedSGD and FedAvg. Then, we explore federated learning under different communication systems, \ie synchronous vs. semi-asynchronous, and provide a summarized overview of the corresponding algorithms.


\subsection{Notations of Federated Learning}

We consider an FL system consists of a set of clients $\mathcal{C} = \{C_1, C_2,...,C_N\}$ and a server $S$. The server has a global model $M_g$ whose weights are denoted as $w_g$ and a collection $\mathcal{S}$ that stores all the data uploaded by the clients. Each client $C_i$ has its own model $M_i$ and dataset $\mathcal{D}_i$ for training, where each data point $k \in \mathcal{D}_i$ is denoted by $(x_k, y_k)$. We denote the size of each dataset as $D_i = |\mathcal{D}_i|$. In addition, each of the clients may use a different optimization method to train its local model, but the model architecture among clients is consistent. We use 
$w_i$ to denote the model parameters and $L_i$ to represent the loss function of the model in $C_i$. Therefore, $C_i$ can use a prediction loss function $l$ to train its local model as:
\begin{equation}
    \min_{w_i} \ L_i(w_i) \triangleq \frac{1}{D_i} \sum_{k \in \mathcal{D}_i} l(k;w_i) = \frac{1}{D_i} \sum_{k \in \mathcal{D}_i} l(y_k, w_i(x_k))
\end{equation}

In particular, if $C_i$ uses mini-batch SGD to optimize the its model with the batch set $\mathcal{B}_i$ at the $e$-th local epoch, the entire training process can be represented by the following equation:
\begin{equation}
\begin{split}
        w_{i,e+1} &= w_{i, e} - \eta_i\nabla L_{i,e} \\ &= w_{i, e} - \frac{\eta_i}{D_i}  \sum_{B_i \in \mathcal{B_i}} \nabla l(w_{i,e}; B_i),
\end{split}
\label{equ:mini-batch}
\end{equation}
where $\eta_i$ is the learning rate of this client. 

Since FL does not prescribe specific optimization algorithms for each client, without loss of generality, we presume that each client employs the mini-batch SGD optimization method in the subsequent discussions in this paper.

\begin{table}[!htp]
    \normalsize
    \caption{Key Notations}
    \centering
    \begin{tabular*}{\linewidth}{c l}
    \hline
       Symbol  & Description \\
    \hline
         $\mathcal{C}$ & the set of clients \\
         $C_i$ & the \textit{i}-th client\\
         $S$ & the server \\
         $\mathcal{S}$ & the set of uploaded data stored on the server  \\
         $w_g$ & parameters of global model \\
         $\mathcal{D}_i$ & the dataset for training in $C_i$ \\
         $D_i$ & the size of $\mathcal{D}_i$ \\
         $w_i$ & parameters of the local model in $C_i$\\
         $L_i$ & the loss function of $w_i$ \\
         $\nabla L_i$ & the gradient of $L_i$ \\
         \multirow{2}*{$K$} & the activation rate in synchronous FL \\
         & the target amount in semi-asynchronous FL \\
         $E$ & the maximum number of local epochs  \\
         $T$ & the maximum number of global epochs \\
         $\eta_i$ & the learning rate of $C_i$ \\
         $\eta$ & the learning rate of $S$ \\
         $B$ & a batch of data \\
         $\mathcal{B}$ & the set of batch data \\
         $\tau_s^t$ & the staleness of the data $s$ in $t$-th global epoch \\
         $Acc_t$ & the target accuracy to evaluate convergence \\
         $ost$ & the oscillation threshold \\
         $T_s$ & the epochs that achieve the target accuracy firstly\\
         $T_f$ & the epochs after which remains stable \\
    \hline
    \end{tabular*}
\end{table}
\subsection{Aggregation Strategies}
In this section, we briefly describe the different aggregation strategies between FedSGD and FedAvg.
\subsubsection{FedSGD}
In FedSGD, the server aggregates model gradients from each client that computes the cumulative gradient while training its local model as:
\begin{equation}
    \nabla L_i = \sum_{e=1}^E L_{i,e} = \frac{1}{D_i}\sum_{e=1}^E \sum_{B_i \in \mathcal{B}_i} \nabla l(w_{i,e}; B_i)
\label{equ:local_accumu_gradient}
\end{equation}

Upon completion of local epoch computations, the client $C_i$ transfers the accumulated gradient $\nabla L_i$ to the server and the server stores it in the collection $\mathcal{S}$. When $\mathcal{S}$ meets specific conditions, the server aggregates all gradients and updates the global model at the $t$-th global epoch according to
\begin{equation}
    \nabla L = \frac{1}{|\mathcal{S}|} \sum_{\nabla L_i \in \mathcal{S}} \nabla L_i 
\label{equ:fedsgd_agg}
\end{equation}

\begin{equation}
    w_g^t = w_g^{t-1} - \eta \nabla L,
\label{equ:fedsgd_update}
\end{equation}
where $\eta$ is the learning rate for the global model training. 

\subsubsection{FedAvg}
In FedAvg, the clients achieve communication efficiency by making multiple local updates before sending their local models to the server, which averages the locally updated models to compute the next round of global model. Under this strategy, the clients upload the weight parameters $w_i$ of their local models to the server instead of accumulated gradients. The server stores all weight parameters in a collection $\mathcal{S}$. Once $\mathcal{S}$ meets certain conditions in the $t$-th global epoch, the server aggregates these parameters to update the global model as performed by:
\begin{equation}
    w_g^{t} = \frac{1}{D} \sum_{w_i \in \mathcal{S}} D_i w_i,
\label{equ:fedavg_update}
\end{equation}
where $D \triangleq \sum_{w_i \in \mathcal{S}} D_i$.

Researchers commonly favor to use FedAvg in synchronous federated learning due to its faster convergence speed. Studies~\cite{melis2019exploiting,zhu2019deep,wainakh2021user,chai2020fedeval} suggest that FedAvg exhibits greater resilience against gradient leakage attacks than FedSGD and offers enhanced privacy protection for clients.

\subsection{Communication Strategies}
Below we outline the differences of communication strategies between synchronous and semi-asynchronous FL.

\begin{figure*}[!t]
\centering
\subfloat[]{\includegraphics[width=3.5in]{pic/SFL.png}%
\label{fig_syn_fl}}
\hfil
\subfloat[]{\includegraphics[width=3.5in]{pic/SAFL.png}%
\label{fig_safl}}
\caption{A comparison between synchronous federated learning and semi-asynchronous federated learning (a) Synchronous Federated Learning. (b) Semi-Asynchronous Federated Learning.}
\label{fig_compare}
\end{figure*}

\subsubsection{Synchronous}
Algorithm~\ref{algo:sfl} provides the detailed process of synchronous FL. 
In each round of synchronous FL, the server randomly selects a set of active clients, denoted by $\mathcal{AC} \subseteq \mathcal{C}$, that occupy a specific proportion of all distributed clients, and leverages local model updates from these active clients to train the global model(Lines 4-5). We refer to the proportion at which the server selects clients as the activation rate, denoted by $K$ that is equal to $|\mathcal{S}|$. The server does not update the global model until it receives shared data from all clients in $\mathcal{AC}$(Lines 6-8). Then, it will broadcast the new model to all clients(Line 9). On the client side, while one client receives a new model, it will replace the local model by it(Line 11) and check whether it's activated(Line 12). If it's activated, this client will start local training(Line 12-19). Otherwise, it has to wait in idle time(Line 21).
    \begin{algorithm}[htbp]
        \caption{Synchronous Federated Learning}
        \label{algo:sfl}
        \begin{algorithmic}[1] 
            \REQUIRE
            \STATE  Initialize the global model and broadcast the task
            \FOR {each global epoch $t$}
                \STATE $\mathcal{S} := \phi$
                \STATE Randomly select active clients with a proportion $K$
                \WHILE{$\exists C_i \in \mathcal{AC}$ has not uploaded the data.}
                \STATE Wait for the end of local training in $C_i$
                \ENDWHILE
                \STATE Aggregate model updates by Eq.~\ref{equ:fedsgd_update} or Eq.~\ref{equ:fedavg_update}
                \STATE Broadcast $w_g^t$ to all clients in $\mathcal{C}$
            \ENDFOR
            %\ENDLOOP
            
            \ENSURE
            \STATE  Update local model by $w_{i,0}:=w_g^{t-1}$
            \IF{the client is activated}
            \STATE Train the local model based on $w_{i,0}$ and Eq.~\ref{equ:mini-batch}
            \IF{the aggregation strategy is FedSGD}
            \STATE Compute the accumulative gradients by Eq.~\ref{equ:local_accumu_gradient}
            \STATE Upload $\nabla L_i$ to Sever $S$
            \ELSE
            \STATE Upload $w_{i,E}$ to Sever $S$
            \ENDIF
            \ELSE
            \STATE Wait in idle time.
            \ENDIF\\
        \end{algorithmic}
    \end{algorithm}

The algorithm implements that the server has a strong control over individual clients by performing a synchronized aggregation of model updates from these clients in synchronous FL. However, the training process can be slow since there exist runtime differences (\eg communication conditions and performance) among active clients. Consequently, some devices may be forced to wait (in idle time) for late-arriving clients (stragglers) such that the server finishes one round of the global model training. This results in a waste of both computational resources and processing time.

\subsubsection{Semi-asynchronous}
We outline the detailed process of semi-asynchronous FL in Algorithm~\ref{algo:safl}. 
Compared to the synchronous counterpart, semi-asynchronous FL provides a better solution to the straggler issue. In the semi-asynchronous scenario, the server does not select a set of active clients to train the global model in each epoch. Instead, the server passively accepts local updates that are uploaded by all clients(Line 4-6). Whenever a sufficient amount of information is received, the server performs an aggregation and deploys the latest global model across distributed clients(Line 7-9). On the client side, each individual device undergoes continuous training(Line 18) and uploads model updates after completing each local epoch without interruption(Line 19-24). If no new global model is received, the client continues training; otherwise, it updates the local model to the latest global model(Line 13-17).



    \begin{algorithm}[htbp]
        \caption{Semi-asynchronous Federated Learning}
        \label{algo:safl}
        \begin{algorithmic}[1] 
            \REQUIRE
            \STATE  Initialize the global model and broadcast the task
            \STATE  $\mathcal{S} := \phi$
            \FOR {each global epoch $t$}
                \WHILE{$|\mathcal{S}| < K$}
                \STATE Wait for the end of local training
                \ENDWHILE
                \STATE Aggregate model by Eq.~\ref{equ:fedsgd_update} or Eq.~\ref{equ:fedavg_update}
                \STATE Broadcast $w_g^t$ to all clients in $\mathcal{C}$
                \STATE Remove the used data in $\mathcal{S}$
            \ENDFOR
            \STATE Broadcast \textbf{END} flag
            
            \ENSURE
            \WHILE{The \textbf{END} flag is not received}
            \IF{there is a new global model $w_g^{t-1}$}
            \STATE $w_{i,0}:=w_g^{t-1}$
            \ELSE
            \STATE $w_{i,0}:=w_{i,E}$
            \ENDIF
            
            \STATE Train the local model based on $w_{i,0}$ and Eq.~\ref{equ:mini-batch}
            \IF{the aggregation strategies is FedSGD}
            \STATE Compute the accumulative gradients by Eq.~\ref{equ:local_accumu_gradient}
            \STATE Upload $\nabla L_i$ to Sever $S$
            \ELSE
            \STATE Upload $w_{i,E}$ to Sever $S$
            \ENDIF
            \ENDWHILE
        \end{algorithmic}
    \end{algorithm}

Semi-asynchronous FL improves the communication efficiency of federated learning by addressing the straggler problem. However, models trained through semi-asynchronous FL typically do not achieve the same quality as those obtained through synchronous FL. Due to the complexity of data distribution in the real world, semi-asynchronous FL can lead to model bias. That said, the global model trained through semi-asynchronous FL fits the data distribution of clients that have faster update speeds better than those with slower speeds.



==> contents/related.tex <==
\section{Related Works}
With the increasing number of users and devices connecting to the Internet of Things (IoT), transmitting data from devices to the cloud for processing incurs high costs and significant latency\cite{ren2019survey}. Moreover, the communication channels are more open, making data and task information vulnerable to eavesdropping, posing significant challenges to user data privacy. In 2017, Google\cite{mcmahan2017communication} introduced the federated learning algorithm, which keeps user data local and aggregates local model gradients to obtain a global model. Federated learning has become a common solution for collaborative learning. 

As the number of IoT devices increases, there may be a significant disparity in computational power among devices. Researchers\cite{wang2020optimize} have proposed asynchronous federated learning techniques to adapt to the complex IoT environment and demonstrated that asynchronous federated learning can achieve linear convergence to global optima for strongly convex problems or non-convex problems with strict constraints. The FedSA algorithm proposed by Ma et al.\cite{ma2021fedsa} addresses the low turnover efficiency and slow convergence speed in federated learning through a semi-asynchronous system. Cheng et al.\cite{cheng2022aafl} applied the asynchronous federated learning model to COVID-19 testing technology, considering the limited resources of medical facilities, and found the optimal resource allocation parameters through optimization problems. Fadlullah\cite{fadlullah2021smart} applied the asynchronous federated learning model in complex scenarios involving space, air, and ground, aggregating ground models from satellites as edge devices, reducing waiting time at ground base stations, and ensuring efficient utilization of local resources. Zhang\cite{zhang2021privacy} considered privacy aspects in the asynchronous federated learning model by grouping clients with the same privacy budget and privacy performance.

==> contents/summary.tex <==
\section{Conclusion}
In this paper, we explored the performance differences of different aggregation targets in synchronous federated learning as well as semi-asynchronous federated learning. Based on extensive experimental results on computer vision tasks and natural language processing tasks, although the aggregation of models and gradients has almost the same effect in synchronous federated learning, this conclusion does not hold in the semi-asynchronous federated learning scenario. $FedSGD$, or gradient aggregation, demonstrates high accuracy in semi-asynchronous federated learning but exhibits poor convergence and significant fluctuations in both model accuracy and loss. On the other hand, $FedAvg$, or model aggregation, shows good convergence and loss stability. However, its convergence speed is slow, leading to a notable difference in model test accuracy compared to gradient aggregation within the same number of communication rounds. This means that in semi-asynchronous federated learning, different aggregation targets introduce a trade-off between model accuracy and convergence. Due to the complexity of the communication environment, we have only conducted a qualitative analysis of this phenomenon in this paper, providing possible reasons for the emergence of this trade-off problem. An apparent future work is to theoretically explain and analyze the causes of this phenomenon.

To the best of our knowledge, this is the first study investigating the impact of aggregation objects in semi-asynchronous federated learning. We believe that this work carries notable implications for future studies on semi-asynchronous federated learning, providing guidance to researchers in meticulously selecting aggregation targets tailored to specific experiment requirements. Additionally, in the exploration of the straggler problem, a judicious choice of aggregation targets can be leveraged to analyze the algorithm's performance. Our code and data are available at: xx

==> tmp/tmp.tex <==
\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.
